Deformable Multibody Modeling for Model Predictive Control in Legged Locomotion with Embodied Compliance

The paper presents a method to stabilize dynamic gait for a legged robot with embodied compliance. Our approach introduces a unified description for rigid and compliant bodies to approximate their deformation and a formulation for deformable multibody systems. We develop the centroidal composite predictive deformed inertia (CCPDI) tensor of a deformable multibody system and show how to integrate it with the standard-of-practice model predictive controller (MPC). Simulation shows that the resultant control framework can stabilize trot stepping on a quadrupedal robot with both rigid and compliant spines under the same MPC configurations. Compared to standard MPC, the developed CCPDI-enabled MPC distributes the ground reactive forces closer to the heuristics for body balance, and it is thus more likely to stabilize the gaits of the compliant robot. A parametric study shows that our method preserves some level of robustness within a suitable envelope of key parameter values.

==> Tables/states_summary.tex <==
\begin{table}[!th]
\vspace{-5pt}
    \caption{Summary of Important Variables} % \protect\footnotemark }
    \vspace{-9pt}
    \label{table:variable_summary}
    \begin{center}
    \renewcommand{\arraystretch}{1.5}
    \begin{tabular}{p{2.5cm}>{\centering}p{2.3cm}>{\centering}p{2.3cm}}% >{\centering}p{1.5cm}}
    %{\columnwidth}{ X X X X}  % @{\hskip 2cm}
        \toprule
        \textbf{Variables} & Dimensional Symbol at $T_k$ & Non-dimensional Symbol at $T_k$ \\ % & $T_2$ \\
        \midrule
        \midrule
        Length or Position
        & $r_k$, $x_k$, $z_k$ 
        & $\Tilde{r}_k$, $\Tilde{x}_k$, $\Tilde{z}_k$ \\ %TODO 
        %\midrule
        Linear Velocity
        & $v_k$, $v_{xk}$, $v_{zk}$ 
        & $\Tilde{v}_k$, $\Tilde{v}_{xk}$, $\Tilde{v}_{zk}$ \\ %TODO 
        %\midrule
        Linear Acceleration
        & $\dot{v}_k$, $\dot{v}_{xk}$, $\dot{v}_{zk}$ 
        & $\Tilde{\dot{v}}_k$, $\Tilde{\dot{v}}_{xk}$, $\Tilde{\dot{v}}_{zk}$ \\ %TODO 
        \midrule
        Angle
        & $\alpha_k$, $\beta_k$, $\gamma_k$, $\theta_k$ 
        & $\Tilde{\alpha}_k$, $\Tilde{\beta}_k$, $\Tilde{\gamma}_k$, $\Tilde{\theta}_k$ \\ %TODO
        %\midrule
        Angular Velocity
        & $\dot{\alpha}_k$, $\dot{\beta}_k$, $\dot{\gamma}_k$,  $\dot{\theta}_k$, $\omega_k$ 
        & $\Tilde{\dot{\alpha}}_k$ $\Tilde{\dot{\beta}}_k$, $\Tilde{\dot{\gamma}}_k$, $\Tilde{\dot{\theta}}_k$, $\Tilde{\omega}_k$ \\ %TODO
        %\midrule
        Angular Acceleration
        & $\ddot{\alpha}_k$, $\ddot{\beta}_k$, $\ddot{\gamma}_k$, $\ddot{\theta}_k$ 
        & $\Tilde{\ddot{\alpha}}_k$, $\Tilde{\ddot{\beta}}_k$, $\Tilde{\ddot{\gamma}}_k$, $\Tilde{\ddot{\theta}}_k$ \\ %TODO
        \bottomrule
        
    \end{tabular}
    \end{center}
    \footnotesize{$\quad$ Note that Figure~\ref{fig:workflow_landing_sequence} defines $T_k,k = 0, 1, 2$.}
    \vspace{-12pt}
\end{table}

%\footnotetext{The parameters are selected based on MIT Cheetah 3~\cite{bledt2018cheetah} for a more realistic physical background. The peak joint torque is set to $0.8 \tau_{max}$ for actuator safety.} 
